Enhancing Local and Global Structure in Compressed AI Agent Memory

AI agents store text as embedding vectors and compress them at scale. A compression is accepted when each item's nearest neighbors survive, but agents also consolidate, delete, and compare memories, tasks that depend on which items lie far apart. We evaluate both ends with two label-free fidelities from our prior work: the local fidelity $L$ at 10 neighbors and the global fidelity $G$ at 30 to 50 percent of the memory. At 96 bytes per passage, rescored binary codes reach an $L$ of 0.97 yet move 10.1 percent of passages to another theme; PCA with 8-bit codes, at an $L$ of 0.77, moves 1.7 percent. Rescoring leaves the stored codes, and thus $G$, unchanged. We prove that across the $G$ band, $1-\nu_k$ is at most 2 to 2.18 times the square root of the near-far rank-violation rate, and that this rate follows the distance noise of the compression (correlation 0.979). Our locality-aware quantization (LAQ) turns the bound into a hinge objective on the codebooks of an OPQ index, keeping its bytes, rotation, and search. To our knowledge, LAQ is the first quantizer whose objective comes from a proven bound on the far end. Reconstruction alone raises $G$ in 0 of 52 held-out runs; the far hinge raises it in all 52. LAQ raises $G$ in all 52 ($p=8.5\times 10^{-4}$ over 13 memory-encoder groups), including the external FinDER memory, has the highest $G$ of seven equal-size quantizers in all 12 Multi-Doc-2025 runs, scales to a million passages, and keeps evidence recall.

==> gen/tab_pred_rows.tex <==
FinQA, BGE-base & same top-10 retrieved & near & 1.00 & 0.89 & 0.99 & 0.30 \\
 & same themes (ARI) & far & 0.80 & 0.90 & 0.04 & 0.68 \\
 & same peer groups & far & 0.87 & 0.83 & 0.53 & 0.26 \\
 & information barrier & far & 0.91 & 0.84 & 0.65 & 0.21 \\
 & company map & far & 0.91 & 0.86 & 0.64 & 0.26 \\
 & sector map & far & 0.86 & 0.84 & 0.45 & 0.35 \\
\addlinespace[2pt]
FinQA, E5-base & same top-10 retrieved & near & 0.98 & 0.94 & 0.94 & 0.78 \\
 & same themes (ARI) & far & 0.83 & 0.93 & 0.01 & 0.76 \\
 & same peer groups & far & 0.89 & 0.90 & 0.45 & 0.51 \\
 & information barrier & far & 0.88 & 0.88 & 0.44 & 0.44 \\
 & company map & far & 0.90 & 0.89 & 0.50 & 0.45 \\
 & sector map & far & 0.89 & 0.87 & 0.52 & 0.37 \\
\addlinespace[2pt]
FinQA, BGE-large & same top-10 retrieved & near & 1.00 & 0.92 & 0.97 & 0.31 \\
 & same themes (ARI) & far & 0.83 & 0.91 & -0.02 & 0.66 \\
 & same peer groups & far & 0.88 & 0.86 & 0.43 & 0.30 \\
 & information barrier & far & 0.90 & 0.88 & 0.48 & 0.32 \\
 & company map & far & 0.94 & 0.91 & 0.63 & 0.34 \\
 & sector map & far & 0.87 & 0.86 & 0.39 & 0.32 \\
\addlinespace[2pt]
FinQA, MobileCLIP2 & same top-10 retrieved & near & 0.95 & 0.92 & 0.83 & 0.70 \\
 & same themes (ARI) & far & 0.77 & 0.90 & 0.02 & 0.74 \\
 & same peer groups & far & 0.88 & 0.90 & 0.49 & 0.63 \\
 & information barrier & far & 0.88 & 0.88 & 0.55 & 0.54 \\
 & company map & far & 0.88 & 0.90 & 0.51 & 0.61 \\
 & sector map & far & 0.73 & 0.83 & 0.11 & 0.57 \\
\addlinespace[2pt]
FinQA, RoBERTa & same top-10 retrieved & near & 0.98 & 0.88 & 0.93 & -0.24 \\
 & same themes (ARI) & far & 0.84 & 0.86 & 0.25 & 0.43 \\
 & same peer groups & far & 0.91 & 0.85 & 0.63 & 0.10 \\
 & information barrier & far & 0.91 & 0.99 & 0.14 & 0.92 \\
 & company map & far & 0.95 & 0.93 & 0.67 & 0.46 \\
 & sector map & far & 0.92 & 0.87 & 0.64 & 0.15 \\
\addlinespace[2pt]
FinQA, GloVe & same top-10 retrieved & near & 0.99 & 0.83 & 0.97 & 0.35 \\
 & same themes (ARI) & far & 0.77 & 0.86 & 0.26 & 0.63 \\
 & same peer groups & far & 0.90 & 0.72 & 0.77 & -0.01 \\
 & information barrier & far & 0.92 & 0.93 & 0.78 & 0.81 \\
 & company map & far & 0.89 & 0.94 & 0.66 & 0.84 \\
 & sector map & far & 0.90 & 0.76 & 0.74 & 0.12 \\
\addlinespace[2pt]
LoCoMo, BGE-base & same top-10 retrieved & near & 0.99 & 0.89 & 0.95 & -0.16 \\
 & same memories deleted & far & 0.87 & 0.97 & -0.11 & 0.86 \\
 & session map & far & 0.89 & 0.97 & 0.10 & 0.82 \\
\addlinespace[2pt]
LoCoMo, E5-base & same top-10 retrieved & near & 0.99 & 0.89 & 0.96 & 0.18 \\
 & same memories deleted & far & 0.87 & 0.90 & 0.36 & 0.55 \\
 & session map & far & 0.90 & 0.98 & 0.36 & 0.92 \\
\addlinespace[2pt]
LoCoMo, BGE-large & same top-10 retrieved & near & 0.99 & 0.90 & 0.97 & -0.35 \\
 & same memories deleted & far & 0.90 & 0.99 & -0.14 & 0.93 \\
 & session map & far & 0.91 & 0.94 & 0.30 & 0.66 \\
\addlinespace[2pt]
LoCoMo, MobileCLIP2 & same top-10 retrieved & near & 1.00 & 0.88 & 0.99 & -0.25 \\
 & same memories deleted & far & 0.88 & 0.96 & 0.19 & 0.84 \\
 & session map & far & 0.86 & 0.92 & 0.22 & 0.67 \\
\addlinespace[2pt]
LoCoMo, RoBERTa & same top-10 retrieved & near & 0.97 & 0.89 & 0.87 & -0.36 \\
 & same memories deleted & far & 0.92 & 0.98 & -0.03 & 0.83 \\
 & session map & far & 0.93 & 0.97 & 0.26 & 0.71 \\
\addlinespace[2pt]
LoCoMo, GloVe & same top-10 retrieved & near & 0.99 & 0.85 & 0.97 & -0.57 \\
 & same memories deleted & far & 0.92 & 0.96 & 0.43 & 0.78 \\
 & session map & far & 0.90 & 0.99 & 0.20 & 0.93 \\
\addlinespace[2pt]
20 Newsgroups, MobileCLIP2 & label precision of 10 neighbors & near & 0.59 & 0.29 & 0.68 & -0.48 \\
 & same memories deleted & far & 0.90 & 0.95 & 0.60 & 0.80 \\
 & same themes (ARI) & far & 0.77 & 0.81 & 0.25 & 0.48 \\
 & topic map & far & 0.68 & 0.79 & 0.03 & 0.56 \\
\addlinespace[2pt]
20 Newsgroups, RoBERTa & label precision of 10 neighbors & near & 0.62 & 0.41 & 0.76 & -0.65 \\
 & same memories deleted & far & 0.92 & 0.98 & -0.06 & 0.85 \\
 & same themes (ARI) & far & 0.91 & 0.88 & 0.53 & 0.12 \\
 & topic map & far & 0.93 & 0.95 & 0.38 & 0.56 \\
\addlinespace[2pt]
20 Newsgroups, GloVe & label precision of 10 neighbors & near & 0.67 & 0.34 & 0.83 & -0.71 \\
 & same memories deleted & far & 0.93 & 0.97 & 0.59 & 0.86 \\
 & same themes (ARI) & far & 0.87 & 0.89 & 0.40 & 0.52 \\
 & topic map & far & 0.80 & 0.88 & 0.09 & 0.61 \\
\addlinespace[2pt]
AG News, MobileCLIP2 & label precision of 10 neighbors & near & 0.31 & 0.49 & -0.26 & 0.47 \\
 & same memories deleted & far & 0.86 & 0.93 & 0.32 & 0.74 \\
 & same themes (ARI) & far & 0.73 & 0.83 & 0.03 & 0.59 \\
\addlinespace[2pt]
AG News, RoBERTa & label precision of 10 neighbors & near & 0.62 & 0.46 & 0.65 & -0.51 \\
 & same memories deleted & far & 0.93 & 0.98 & 0.03 & 0.83 \\
 & same themes (ARI) & far & 0.86 & 0.85 & 0.32 & 0.21 \\
\addlinespace[2pt]
AG News, GloVe & label precision of 10 neighbors & near & 0.24 & 0.22 & 0.10 & 0.04 \\
 & same memories deleted & far & 0.86 & 0.95 & 0.42 & 0.85 \\
 & same themes (ARI) & far & 0.62 & 0.80 & -0.14 & 0.65 \\
\addlinespace[2pt]


==> gen/tab_runs.tex <==
\begin{tabular}{@{}lllcccc@{}}
\toprule
Memory & Encoder & Split & $G$ OPQ & $G$ LAQ & $L$ OPQ & $L$ LAQ \\
\midrule
FinQA & BGE-base & 2026 & 0.7927 & 0.8021 & 0.8537 & 0.8566 \\
 &  & 2027 & 0.7930 & 0.8020 & 0.8579 & 0.8570 \\
 &  & 2028 & 0.7885 & 0.7951 & 0.8534 & 0.8557 \\
 &  & 2029 & 0.7958 & 0.8035 & 0.8489 & 0.8514 \\
 & E5-base & 2026 & 0.7872 & 0.7959 & 0.8413 & 0.8458 \\
 &  & 2027 & 0.7858 & 0.7952 & 0.8463 & 0.8544 \\
 &  & 2028 & 0.7781 & 0.7884 & 0.8440 & 0.8486 \\
 &  & 2029 & 0.7867 & 0.7944 & 0.8469 & 0.8450 \\
 & BGE-large & 2026 & 0.8227 & 0.8280 & 0.8819 & 0.8840 \\
 &  & 2027 & 0.8209 & 0.8261 & 0.8844 & 0.8869 \\
 &  & 2028 & 0.8185 & 0.8260 & 0.8884 & 0.8910 \\
 &  & 2029 & 0.8266 & 0.8342 & 0.8879 & 0.8880 \\
\midrule
LoCoMo & BGE-base & 2026 & 0.8667 & 0.8744 & 0.8186 & 0.8224 \\
 &  & 2027 & 0.8572 & 0.8641 & 0.8349 & 0.8358 \\
 &  & 2028 & 0.8319 & 0.8440 & 0.8148 & 0.8182 \\
 &  & 2029 & 0.8722 & 0.8777 & 0.8319 & 0.8302 \\
 & E5-base & 2026 & 0.7979 & 0.8043 & 0.7651 & 0.7671 \\
 &  & 2027 & 0.7681 & 0.7785 & 0.7859 & 0.7946 \\
 &  & 2028 & 0.7703 & 0.7807 & 0.7612 & 0.7697 \\
 &  & 2029 & 0.8072 & 0.8156 & 0.7825 & 0.7806 \\
 & BGE-large & 2026 & 0.8921 & 0.8994 & 0.8496 & 0.8574 \\
 &  & 2027 & 0.8928 & 0.8989 & 0.8813 & 0.8790 \\
 &  & 2028 & 0.8678 & 0.8759 & 0.8522 & 0.8518 \\
 &  & 2029 & 0.9128 & 0.9175 & 0.8587 & 0.8602 \\
\midrule
Multi-Doc & BGE-base & 2026 & 0.8196 & 0.8306 & 0.8132 & 0.8183 \\
 &  & 2027 & 0.8140 & 0.8266 & 0.8181 & 0.8208 \\
 &  & 2028 & 0.8274 & 0.8381 & 0.8102 & 0.8122 \\
 &  & 2029 & 0.8165 & 0.8271 & 0.8183 & 0.8207 \\
 & E5-base & 2026 & 0.8154 & 0.8320 & 0.8018 & 0.8092 \\
 &  & 2027 & 0.8154 & 0.8290 & 0.8068 & 0.8122 \\
 &  & 2028 & 0.8167 & 0.8302 & 0.7944 & 0.7999 \\
 &  & 2029 & 0.8140 & 0.8282 & 0.8037 & 0.8132 \\
 & BGE-large & 2026 & 0.8552 & 0.8647 & 0.8526 & 0.8572 \\
 &  & 2027 & 0.8540 & 0.8635 & 0.8564 & 0.8601 \\
 &  & 2028 & 0.8608 & 0.8686 & 0.8462 & 0.8524 \\
 &  & 2029 & 0.8545 & 0.8617 & 0.8557 & 0.8559 \\
 & Titan V2 & 2026 & 0.6680 & 0.7025 & 0.7942 & 0.8010 \\
 &  & 2027 & 0.6434 & 0.6811 & 0.7962 & 0.8043 \\
 &  & 2028 & 0.6651 & 0.7030 & 0.7848 & 0.7958 \\
 &  & 2029 & 0.6480 & 0.6803 & 0.7852 & 0.7909 \\
\rawinput{gen/tab_runs_finder.tex}
\bottomrule
\end{tabular}


==> gen/tab_runs_finder.tex <==
\midrule
FinDER & BGE-base & 2026 & 0.8139 & 0.8303 & 0.8046 & 0.8072 \\
 &  & 2027 & 0.8142 & 0.8312 & 0.8024 & 0.8055 \\
 &  & 2028 & 0.8142 & 0.8305 & 0.8029 & 0.8069 \\
 &  & 2029 & 0.8137 & 0.8289 & 0.8049 & 0.8076 \\
 & E5-base & 2026 & 0.7982 & 0.8157 & 0.7809 & 0.7893 \\
 &  & 2027 & 0.8028 & 0.8202 & 0.7793 & 0.7854 \\
 &  & 2028 & 0.8075 & 0.8238 & 0.7812 & 0.7883 \\
 &  & 2029 & 0.8032 & 0.8200 & 0.7842 & 0.7905 \\
 & BGE-large & 2026 & 0.8456 & 0.8559 & 0.8450 & 0.8480 \\
 &  & 2027 & 0.8458 & 0.8558 & 0.8445 & 0.8494 \\
 &  & 2028 & 0.8461 & 0.8563 & 0.8433 & 0.8478 \\
 &  & 2029 & 0.8439 & 0.8567 & 0.8393 & 0.8454 \\

